Linear-Time Algorithms for k-Edge-Connected Components, k-Lean Tree Decompositions, and More

We present $k^{O(k^2)} m$ time algorithms for various problems about decomposing a given undirected graph by edge cuts or vertex separators of size $<k$ into parts that are ``well-connected'' with respect to cuts or separators of size $<k$; here, $m$ is the total number of vertices and edges of the graph. As an application of our results, we obtain for every fixed $k$ a linear-time algorithm for computing the $k$-edge-connected components of a given graph, solving a long-standing open problem. More generally, we obtain a $k^{O(k^2)} m$ time algorithm for computing a $k$-Gomory-Hu tree of a given graph, which is a structure representing pairwise minimum cuts of size $<k$. Our main technical result, from which the other results follow, is a $k^{O(k^2)} m$ time algorithm for computing a $k$-lean tree decomposition of a given graph. This is a tree decomposition with adhesion size $<k$ that captures the existence of separators of size $<k$ between subsets of its bags. A $k$-lean tree decomposition is also an unbreakable tree decomposition with optimal unbreakability parameters for the adhesion size bound $k$. As further applications, we obtain $k^{O(k^2)} m$ time algorithms for $k$-vertex connectivity and for element connectivity $k$-Gomory-Hu tree. All of our algorithms are deterministic. Our techniques are inspired by the tenth paper of the Graph Minors series of Robertson and Seymour and by Bodlaender's parameterized linear-time algorithm for treewidth.

==> Preamble.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}
\pdfoutput=1

\usepackage{microtype}
\usepackage{mdframed}
\usepackage{csquotes}
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{soul}
\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}
\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amssymb}
\usepackage{amstext}
\usepackage{graphicx,tikz-cd}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{graphics}
\usepackage{pgf}
\usepackage{paralist} 
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
\usepackage{todonotes}
%%%%%
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{enumitem}
\usepackage{makecell}
\usepackage{thmtools, thm-restate}
\usepackage{thm-autoref}
 \usepackage{mathdots}
%\usepackage{wrapfig}
\usepackage{multirow}
%\usetikzlibrary{cd}
\usepackage{chngcntr}
\usepackage{apptools}
\usepackage{accents}
\AtAppendix{\counterwithin{lemma}{section}}

  


\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\numberwithin{equation}{section}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{hypothesis}[equation]{Hypothesis}
\newtheorem{claim}[equation]{Claim}
\newtheorem{definition}[equation]{Definition}
\newtheorem{observation}[equation]{Observation}
\newtheorem{proposition}[equation]{Proposition}
\newtheorem{corollary}[equation]{Corollary}
\newtheorem{mainlemma}[equation]{Main lemma}
%\newtheorem{redrule}[lemma]{Reduction Rule}
%\newtheorem{remark}[lemma]{Remark}
%\newtheorem{reduction}[lemma]{Reduction Rule}
%\newtheorem{conjecture}[lemma]{Conjecture}
\newcommand{\cqed}{\ensuremath{\lhd}}
\makeatletter
\newenvironment{claimproof}{\par
  \pushQED{\cqed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item\relax
  {\itshape
    Proof of the claim\@addpunct{.}}\hspace\labelsep\ignorespaces
}{%
  \hfill\popQED\endtrivlist\@endpefalse
}
\makeatother


\date{}


\usepackage{booktabs}

\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hypertexnames = false,
                 hyperfigures
                 ]{hyperref}

\usepackage[nameinlink]{cleveref}
\crefname{observation}{Observation}{Observations}
\crefname{claim}{Claim}{Claims}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\crefname{mainlemma}{Main lemma}{Main lemmas}




\newcommand{\OO}{\mathcal{O}}
\DeclareMathOperator{\polylog}{polylog}

%Define in defs
\newcommand{\primal}{\mathcal{P}}
\newcommand{\bd}{\mathsf{bd}}
\newcommand{\bdc}{\lambda}
\newcommand{\co}[1]{\overline{#1}}
\newcommand{\rank}{\mathsf{rk}}

\newcommand{\bag}{\textsf{bag}}
\newcommand{\flow}{\textsf{flow}}
\newcommand{\flowp}{\textsf{flow}^*}
\newcommand{\cc}{\texttt{cc}}
\newcommand{\adh}{\mathsf{adh}}
\newcommand{\adhsize}{\mathsf{adhsize}}

\newcommand{\contr}{/}
\newcommand{\hyperg}{\mathcal{H}}


\newcommand{\rescliqs}{\triangleleft}
\newcommand{\orescliqs}{\triangleright}


\newcommand{\ninc}{N^{\mathsf{inc}}}


\newcommand{\children}{\mathsf{children}}
\newcommand{\troot}{\mathsf{root}}
\newcommand{\parent}{\mathsf{parent}}

\newcommand{\vint}{V_{\mathsf{int}}}
\newcommand{\eint}{E_{\mathsf{int}}}


%TODO, define in defs: 

\newcommand{\resgcliqs}{\diamond}





\newcommand{\lmap}{\mathcal{L}}
\newcommand{\leafs}{L}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\torso}{\mathsf{torso}}


\newcommand{\runtime}{\mathsf{RT}}
\newcommand{\oruntime}{\mathsf{ORT}}


%Define in Bodlaender section
\newcommand{\elim}{*}


%Define in superbd editing section
\newcommand{\refiset}{\mathfrak{T}}
\newcommand{\compset}{\mathfrak{C}}

% Define in the section about tangles
\newcommand{\bw}{\mathsf{bw}}
\newcommand{\tang}{\mathscr{T}}


% TODO: define
\newcommand{\prop}{\Pi}


% Random
\newcommand{\wilog}{without loss of generality\xspace}


% For lean
\newcommand{\pull}{\mathsf{pull}}
\newcommand{\forget}{\mathsf{forget}}
\newcommand{\paths}{\mathscr{P}}
